Bounds on the spectral radius of real-valued non-negative Kernels on measurable spaces

In this short technical note, we extend a recently published result [Liao2017] on the Perron root (or the spectral radius) of non-negative matrices to real-valued non-negative kernels on an arbitrary measurable space $(\mathrm{E}, \mathcal{E})$. To be precise, for any real-valued non-negative kernel $K : \mathrm{E}\times \mathcal{E} \rightarrow \mathbb{R}$, we prove that the spectral radius $\rho(K)$ of $K$ satisfies $$ \inf_{x \in \mathrm{E} } \frac{ \mathcal{R} K \cdotp L (x) }{ \mathcal{R} L (x) } \le \rho(K) \le \sup_{x \in \mathrm{E} } \frac{ \mathcal{R} K\cdotp L (x) }{ \mathcal{R} L (x) }, $$ where $L$ is an arbitrary Kernel on $(\mathrm{E}, \mathcal{E})$, which is integrable with respect to the left eigenmeasure of $K$ and satisfies $ \mathcal{R} L (x) >0 $ for all $x \in \mathrm{E}$, and the operator $\mathcal{R}$ is defined by $\mathcal{R}L (x) :=\int_{\mathrm{E}} L(x, \mathrm{d}y) $.

==> Sections/Applications.tex <==


\section{Applications}
\subsection{General branching processes}

for studying the asymptotic behaviour of a general branching process... Harris' book on branching processes...

\subsection{On-off queueing systems}
Markov modulated on-off queueing systems... mention that the decay rate is the Perron root of a transform fo the transition probability matrix... 


==> Sections/Discussions.tex <==
\section{Discussions}
\label{sec:discussions}


==> Sections/Main_result.tex <==

\section{Main result}
\label{sec:main_result}
% \citet{LIAO2017Perron} \citet{Harris1963Branching}

\subsection{Notational conventions}
The following notational conventions are adhered to throughout this technical report. We denote the set of natural numbers and the set of real numbers  by $\setOfNaturals$   and $\setOfReals$ respectively. Let  $\setOfNonnegativeIntegers \defeq \setOfNaturals \cup \{0\}$. For $N \in \setOfNaturals$, let $\setN{N} \defeq \{1,2,\ldots, N \}$. The set of non-negative real numbers is denoted by $\setOfPositiveReals$.  For $A \subseteq \setOfReals$, we denote the Borel $\sigma$-field of subsets of $A$ by $\borel{A}$. For any $f: \setOfReals \rightarrow \setOfReals$, we denote the effective domain of $f$ by $\effectiveDomain{f}$, \ie, $\effectiveDomain{f} \defeq \{ x \in \setOfReals \mid \lvert f(x) \rvert < \infty \}$. For an event $A$, we denote the indicator function of $A$ by $\indicator{A}$, taking value unity when $A$ is true and zero otherwise.

\subsection{Bounds on the Perron root}
Let $(\mathrm{E}, \mathcal{E})$ be a given measurable space. The set $\mathrm{E}$ need not be countable. We assume $\mathrm{E}$ is  a complete and separable metric space.   Denote the space of real-valued non-negative Kernels on $(\mathrm{E}, \mathcal{E})$ by $\mathrm{K}_{\mathrm{E}}$, \ie,
$\mathrm{K}_{\mathrm{E}} \defeq \{ f : \mathrm{E}\times \mathcal{E} \rightarrow \setOfPositiveReals \}$. Given $K \in \mathrm{K}_{\mathrm{E}}  $, define the   operator $  \mathcal{R} K $ as
\begin{align}
  \mathcal{R} K(x) \defeq   \int_{\mathrm{E}} K(x, \differential{y})  \eqstop
  \label{eq:row_sum}
\end{align}
The operator $ \mathcal{R} K$ is analogous to the row sum in the finite case, \ie, when $\mathrm{E}$ is finite and $K$ is  a real matrix. We are interested in getting upper and lower bounds on the largest eigenvalue  $\rho(K)$ of the kernel~$K$. We call $\rho(K)$ the Perron root or the spectral radius of $K$.  Before presenting our main result, we have the following two lemmas.

\begin{myLemma}
Suppose $f : \mathrm{E} \rightarrow \setOfPositiveReals$ and $g :\mathrm{E} \rightarrow \setOfPositiveReals$ are such that $\effectiveDomain{f}=\effectiveDomain{g}=\mathrm{E}$ and $ \int_{\mathrm{E}}  f \differential{ \mu } < \infty,  \int_{\mathrm{E}}  g \differential{ \mu } < \infty $. Then, given a measure~$\mu$ on $\mathrm{E} $,
\begin{align}
  \inf_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) }  \le \frac{ \int_{\mathrm{E}}  f \differential{ \mu }   }{ \int_{\mathrm{E}}  g \differential{\mu} }   \le   \sup_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) } \eqstop
\end{align}
\label{lemma:lemma1}
\end{myLemma}

\begin{proof}[Proof of Lemma~\ref{lemma:lemma1}]
Note that
\begin{align*}
 \frac{ \int_{\mathrm{E}}  f \differential{ \mu }   }{ \int_{\mathrm{E}}  g \differential{\mu} }   =  \frac{ 1 }{ \int_{\mathrm{E}}  g \differential{\mu} }   \int_{\mathrm{E}}  \frac{f}{g} g \differential{ \mu }  
 = \int_{\mathrm{E}}  \frac{f}{g}  \differential{ \nu }   \eqcomma
\end{align*}
where the probability measure $\nu$ on $(\mathrm{E}, \mathcal{E})$ is defined by
\begin{align*}
  \nu (A) \defeq \frac{ 1 }{ \int_{\mathrm{E}}  g \differential{\mu} }   \int_{\mathrm{A}}  g \differential{\mu} , \text{ for } A \in \mathcal{E}  \eqstop
\end{align*}
Note that,
\begin{align*}
   \int_{\mathrm{E}}  \frac{f}{g}  \differential{ \nu }   \ge {} & \inf_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) }  \int_{\mathrm{E}}  \differential{ \nu }  =  \inf_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) } \nu(\mathrm{E})  = \inf_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) }  \eqcomma \\
\text{and } \int_{\mathrm{E}}  \frac{f}{g}  \differential{ \nu }   \le {} & \sup_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) }  \int_{\mathrm{E}}  \differential{ \nu }   =  \sup_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) } \nu(\mathrm{E}) = \sup_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) } \eqstop
\end{align*}
Therefore, we get
\begin{align}
  \inf_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) }  \le \frac{ \int_{\mathrm{E}}  f \differential{ \mu }   }{ \int_{\mathrm{E}}  g \differential{\mu} }   \le   \sup_{x \in \mathrm{E}  } \frac{ f(x) }{  g (x) } \eqstop
\end{align}

%\tdWasiur[]{check if we need any restriction on $\mu$}
\end{proof}

Next we define the product of two kernels on the measurable space $(\mathrm{E}, \mathcal{E})$. Let $F$, and $ G$ be two kernels on $(\mathrm{E}, \mathcal{E})$. Analogous to matrix multiplication, define the new kernel $F \cdotp G  :   \mathrm{E}\times \mathcal{E} \rightarrow   \setOfReals  \cup \{ \infty, - \infty \} $ as
\begin{align}
 F \cdotp  G    (x, A) \defeq \int_{\mathrm{E}}  F(x, \differential{y} )   G(y, A) \eqstop
\end{align}
The next lemma concerns the row sums of the product of two kernels.

\begin{myLemma}
Let $F$, and $ G$ be two kernels on $(\mathrm{E}, \mathcal{E})$ such that $\effectiveDomain{   \mathcal{R}  F \cdotp  G  }=\mathrm{E}$. Then,
\begin{align}
  \mathcal{R}  F \cdotp  G  (x) = \int_{ \mathrm{E}  } F( x, \differential{y} ) \mathcal{R} G(y)  \eqstop
\end{align}
\label{lemma2}
\end{myLemma}

\begin{proof}[Proof of Lemma~\ref{lemma2}]
  Note that,
\begin{align*}
  \mathcal{R}  F \cdotp  G  (x) = {} &  \int_{ \mathrm{E}  }    F \cdotp  G   (x, \differential{z}) \\
  = {} &  \int_{ \mathrm{E}  }  \int_{\mathrm{E}}  F(x, \differential{y} )   G(y,  \differential{z} )  \\
  ={} &  \int_{ \mathrm{E}  }  F(x, \differential{y} )  \int_{\mathrm{E}}    G(y,  \differential{z} )  \\
  ={} &   \int_{ \mathrm{E}  }  F(x, \differential{y} )   \mathcal{R} G(y)   \eqstop
\end{align*}

This completes the proof.

\end{proof}

Now we present our main result on the Perron root $\rho(K)$ of $K$.

\begin{myTheorem}
Let $K$ be a real-valued non-negative kernel, \ie,  $K \in \mathrm{K}_{\mathrm{E}}$.  Let $L$ be an arbitrary kernel on $(\mathrm{E}, \mathcal{E})$, which is not necessarily in $ \mathrm{K}_{\mathrm{E}}$, but satisfies $ \mathcal{R} L (x) >0 $ for all $x \in \mathrm{E}$ and is integrable with respect to the left eigenmeasure of $K$. Then,
\begin{align*}
  \inf_{x \in \mathrm{E}  } \frac{ \mathcal{R} K \cdotp L (x) }{  \mathcal{R} L (x) } \le \rho(K) \le   \sup_{x \in \mathrm{E}  } \frac{ \mathcal{R} K \cdotp L (x) }{  \mathcal{R} L (x) } \eqstop
\end{align*}
\label{thm:mainTheorem}
\end{myTheorem}

\begin{proof}[Proof of Theorem~\ref{thm:mainTheorem}]
Let $r_{K} :\mathrm{E} \rightarrow \setOfReals  $ and $l_{K} : \mathcal{E} \rightarrow \setOfPositiveReals  $ be respectively the right eigenfunction and the left eigenmeasure of $K$ associated with $\rho(K)$. That is,
\begin{align*}
\rho(K)  r_{K}(x)  = {}& \int_{\mathrm{E}} K(x, \differential{y} )   r_{K}(y) \eqcomma   \forall   x \in \mathrm{E}  \eqcomma \\
\rho(K)  l_{K}(A)  ={} &   \int_{\mathrm{E}}   l_K(\differential{x})   K( x, A )  \eqcomma  \forall  A \in \mathcal{E} \eqstop
\end{align*}
Note that $\rho(K)$ is the largest simple eigenvalue of $K$. The existence of $\rho(K),   l_K$, and $r_K$ are guaranteed by  \cite[Theorem III.10.1]{Harris1963Branching}.




 Let $L$ be an arbitrary kernel on $(\mathrm{E}, \mathcal{E})$, which is not necessarily in $ \mathrm{K}_{\mathrm{E}}$, but satisfies $ \mathcal{R} L (x) >0 $ for all $x \in \mathrm{E}$ and is integrable with respect to $l_{K}$ as a measure on $\mathrm{E}$. Then, by the definition of the left eigenmeasure $l_K$, we have
\begin{align*}
    \int_{\mathrm{E}}  l_K(\differential{x})  K( x,  \differential{y}  )   ={} &  \rho(K)  l_{K}(  \differential{y} )  \\
    \implies   \int_{\mathrm{E}}   \mathcal{R} L (y)      \int_{\mathrm{E}}  l_K(\differential{x})  K( x,  \differential{y}  )   ={} &  \rho(K)  \int_{\mathrm{E}}  l_{K}(  \differential{y} )    \mathcal{R} L (y)       \\
    \implies  \int_{\mathrm{E}}  l_K(\differential{x})   \int_{\mathrm{E}}  K( x,  \differential{y}  )   \mathcal{R} L (y)    ={} &  \rho(K)  \int_{\mathrm{E}}  l_{K}(  \differential{y} )   \mathcal{R} L (y) \\
    \implies  \int_{\mathrm{E}}  l_K(\differential{x})     \mathcal{R}  K \cdotp  L  (x)  ={} &  \rho(K)  \int_{\mathrm{E}}  l_{K}(  \differential{y} )   \mathcal{R} L (y) \eqcomma
\end{align*}
because $  \mathcal{R}  K \cdotp  L (x) = \int_{ \mathrm{E}  } K( x, \differential{y} ) \mathcal{R} L(y)  $, by Lemma~\ref{lemma2}. Therefore we have
\begin{align*}
   \rho(K)  ={} & \frac{   \int_{\mathrm{E}}  l_K(\differential{x})     \mathcal{R}  K \cdotp  L  (x)    }{ \int_{\mathrm{E}}  l_{K}(  \differential{x} )   \mathcal{R} L (x) }  \eqstop
\end{align*}
Choosing $\mu = l_K$, $f = \mathcal{R}  K \cdotp  L    $, and $g =   \mathcal{R} L $ in Lemma~\ref{lemma:lemma1}, we get
\begin{align}
  \inf_{x \in \mathrm{E}  } \frac{ \mathcal{R} K \cdotp L (x) }{  \mathcal{R} L (x) } \le \rho(K) \le   \sup_{x \in \mathrm{E}  } \frac{ \mathcal{R} K \cdotp L (x) }{  \mathcal{R} L (x) } \eqstop
\end{align}
This completes the proof.

%\tdWasiur[]{should last inf and sup  be over x where $l_K$ doesn't vanish??}



\end{proof}


% \tdWasiur[]{existence of the Perrot root is guaranteed by \citet[Theorem III.10.1]{Harris1963Branching}   }


==> Sections/Related_work.tex <==
\section{Related work}
\label{sec:related_work}

